Fairly Wired: Towards Leximin-Optimal Division of Electricity

In many parts of the world - particularly in developing countries - the demand for electricity exceeds the available supply. In such cases, it is impossible to provide electricity to all households simultaneously. This raises a fundamental question: how should electricity be allocated fairly? In this paper, we explore this question through the lens of egalitarianism - a principle that emphasizes equality by prioritizing the welfare of the worst-off households. One natural rule that aligns with this principle is to maximize the egalitarian welfare - the smallest utility across all households. We show that computing such an allocation is NP-hard, even under strong simplifying assumptions. Leximin is a stronger fairness notion that generalizes the egalitarian welfare: it also requires to maximize the smallest utility, but then, subject to that, the second-smallest, then the third, and so on. The hardness results extends directly to leximin as well. Despite this, we present a Fully Polynomial-Time Approximation Scheme (FPTAS) for leximin in the special case where the network connectivity graph is a tree. This means that we can efficiently approximate leximin - and, in particular, the egalitarian welfare - to any desired level of accuracy.

==> includes-and-macros.tex <==
\usepackage[utf8]{inputenc}

\usepackage{amsmath,amsthm,amssymb}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{theorem*}{Theorem}
\newtheorem*{lemma*}{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{observation}[theorem]{Observation}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]


\DeclareMathOperator*{\argmax}{arg\,max}

\usepackage{algcompatible}
\usepackage{algorithm}

\usepackage{mathtools}
\usepackage{mathrsfs}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}


\usepackage[dvipsnames]{xcolor}

\usepackage{blindtext}
\usepackage{hyperref}

\usepackage{csquotes}
\usepackage{array}

\usepackage[normalem]{ulem}


\ifdefined\DRAFT
	\newcommand{\er}[1]{\textcolor{blue}{#1}}
	\newcommand{\erel}[1]{\er{(Erel says: #1)}}
	\newcommand{\eden}[1]{\textcolor{red}{(Eden says: #1)}}
	\newcommand{\emark}[1]{\textcolor{red}{ #1}}
	\newcommand{\yon}[1]{\textcolor{Green}{(Yonatan says: #1)}}
     \newcommand{\yonatan}[1]{\textcolor{Green}{(Yonatan says: #1)}}
\else
	\newcommand{\er}[1]{#1}
	\newcommand{\erel}[1]{}
	\newcommand{\eden}[1]{}
	\newcommand{\emark}[1]{#1}
	\newcommand{\yon}[1]{}
\fi


 \newcommand{\valBy}[2]{u_{#1}^{\uparrow}(#2)}

 \newcommand{\forXinY}[2]{ #1 = 1, \ldots, #2}

 
% \renewcommand{\labelenumii}{\arabic{enumi}.\arabic{enumii}}
% \renewcommand{\labelenumiii}{\arabic{enumi}.\arabic{enumii}.\arabic{enumiii}}
% \renewcommand{\labelenumiv}{\arabic{enumi}.\arabic{enumii}.\arabic{enumiii}.\arabic{enumiv}}


\newcommand{\parentOf}[1]{p(#1)}
\newcommand{\maxIndexChildOf}[1]{c(#1)}


\newcommand{\multError}{\alpha}
\newcommand{\equWithExp}[2]{#2 && (#1)}
